rFaaS: Enabling High Performance Serverless with RDMA and Leases

High performance is needed in many computing systems, from batch-managed supercomputers to general-purpose cloud platforms. However, scientific clusters lack elastic parallelism, while clouds cannot offer competitive costs for high-performance applications. In this work, we investigate how modern cloud programming paradigms can bring the elasticity needed to allocate idle resources, decreasing computation costs and improving overall data center efficiency. Function-as-a-Service (FaaS) brings the pay-as-you-go execution of stateless functions, but its performance characteristics cannot match coarse-grained cloud and cluster allocations. To make serverless computing viable for high-performance and latency-sensitive applications, we present rFaaS, an RDMA-accelerated FaaS platform. We identify critical limitations of serverless - centralized scheduling and inefficient network transport - and improve the FaaS architecture with allocation leases and microsecond invocations. We show that our remote functions add only negligible overhead on top of the fastest available networks, and we decrease the execution latency by orders of magnitude compared to contemporary FaaS systems. Furthermore, we demonstrate the performance of rFaaS by evaluating real-world FaaS benchmarks and parallel applications. Overall, our results show that new allocation policies and remote memory access help FaaS applications achieve high performance and bring serverless computing to HPC.

==> secs/apps.tex <==
\label{sec:apps}


\toolname{} can provide significant performance boosts to
applications.
%
The guiding principle --- the application never waits for remote invocations to finish --- is achieved by dividing the work such that the round trip time of invocations
and the time they are executed are hidden by local work.
%
Fine-grained invocations allow developers many opportunities to accelerate their applications.
%
Consequently, the low-latency invocations are critical for such tasks,
and latency plays a part
in deciding what can be safely offloaded to \toolname{}.
%

%Throughout this section, we use an analytical model to estimate the overheads
We use an analytical model to estimate the overheads
of \emph{warm} and \emph{hot} invocations in \toolname, based on prior work of \emph{LogP}~\cite{10.1145/155332.155333} and \emph{LogfP}~\cite{hoefler-pmeo-06}
models. The network performance is expressed with parameters such as latency,
CPU overhead on the sender and receiver, and gap factor. %determining the minimum time between messages.
%
By learning the network parameters, estimating the remote function execution time,
and measuring the \toolname{} overheads (Section~\ref{sec:evaluation}),
we model the round-trip invocation time.

%
We design a model to decide \emph{when} remote invocations can be integrated into HPC
applications, 
%
then show \emph{how} to use \toolname{} as an accelerator for HPC problems.
%
We provide examples of applications and benchmarks that are either a natural
fit or can be adapted to use \toolname{} to offload some of their work.
%
This list is not exhaustive but provides an intuition on using \toolname{} efficiently in practice.


%We use the ping-pong LogGP model, where a single client sends messages to multiple recipients in parallel,
%and modify it accordingly for RDMA data transmissions.
%
%\todo{UPDATE for loggp}
%Given the submission overhead on $P$ processors $o(P)$, the latencies $L_i, L_o$ of transmitting
%input and output of the function, respectively, and the function execution time $T$,
%we design the round-trip invocation model expressing the \toolname overheads $O_h, O_w$
%of hot and warm invocations, respectively:
%\begin{equation}
%  o(P) + L_{i} + O_{\{h,w\}} + T + L_{o}
%\label{eq:perf_model}
%\end{equation}

%\begin{equation}
% \underbrace{o + G \cdot S_i + (P-1)max(o,G\cdot S_i)}_{\text{Dispatch}} + \underbrace{ O_{\{h,w\}} + T }_{\text{Processing}} + \underbrace{o + S_o\cdot G + L }_{\text{Reply}}
%\label{eq:perf_model}
%\end{equation}
%\todo{too complicated and unnecessary in my opinion. I would cut the logp part our completely.}
% %
% In Section \todos{FIXME}, we conduct an empirical verification of the model,
% gaining insights into the scalability of \toolname on large-scale invocations and with large payloads.

% \begin{table}[t]
% \footnotesize
% \vspace{-1.0em}
% \begin{tabular}{lccccccc}
% \textbf{Model} & \textbf{o} \textit{us} & \textbf{L} \textit{us} & \textbf{g} \textit{us} & \textbf{G} \textit{us/MB} & \textbf{O$_h$} \textit{us}  & \textbf{O$_w$} \textit{us} & \textbf{T} \textit{us} \\
% \toprule
% %LogfP          &   0.1307      & 3.3585          & 0           &  -                 &  ???             &  ???            &  ??? \\   
% LogGP          &   0.1307      & 3.2733          & 0           &  87.296            &  ???             &  ???            &  ??? \\   
% \bottomrule
% \end{tabular}
% \caption{Model parameters on our system.}
% \vspace{-3.0em}
% \label{tbl:params}
% \end{table}

%\todo{this is what I would make into an equation, or optionally the version with Nremote. - and reference it with eqoffload}
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
% NEGATIVE VSPACE
\ifcnf
\vspace{-0.75em}
\fi
\paragraph{Massively parallel applications.}
%
These applications are extremely malleable and can therefore make efficient use of \toolname{}.
%
A solver for the Black-Scholes equation~\cite{10.1080/00207160.2012.690865} is a good example,
as it generates many independent tasks of comparable runtime.
%
Assuming we want to achieve the best possible performance, we measure the runtime of one
task $T_{local}$ and then compare this to the runtime $T_{inv}$ of one invocation
using \toolname{}, to which we add the round-trip network time $L$. %of sending the task and receiving the result $L$.
%
There exists a number $N_{local}$ of tasks such that:
%
%\vspace{-0.5em}
\begin{equation}
N_{local} \cdot T_{local} \ge T_{inv}  + L
\label{eq:offload}
\end{equation}
%\vspace{-0.5em}
%
Therefore, if the number of tasks is greater than $N_{local}$, up to $N_{remote}$ tasks can be safely
computed using \toolname{} without incurring any waiting time.
%
$N_{remote}$ is determined as the number of tasks necessary to saturate the available bandwidth $B$:
$\frac{B}{Data_{inv}}$.
%\begin{equation}
%N_{remote} = \frac{B}{Data_{inv}}
%\end{equation}
%
%Should more than $N_{local} + N_{remote}$ tasks be available, for each additional $N_{local}$
%tasks computed locally, up to $N_{remote}$ tasks can be safely offloaded without incurring wait time.
%
Therefore, the throughput of the system only depends on the network link bandwidth,
and the amount of work available to \toolname{}.

% NEGATIVE VSPACE
\ifcnf
\vspace{-0.75em}
\fi
\paragraph{Task-based applications with no sharing within tasks.}
Task-based applications are programs that consist of a series of tasks that must be executed, where some tasks can depend on the results of others, inducing a  task dependency graph~\cite{10.1145/3018743.3018770} - basically a graph stating the order in which tasks must be executed. Task-based applications can profit from \toolname{}, as Eq.~\ref{eq:offload} still holds in this case.
%
However, the number of tasks that 
can be offloaded at any time depends on the width of the task dependency graph at that time - the wider the graph, the more parallelism is exposed, and therefore more tasks can be transferred to \toolname.
%We focus on a benchmarks from the Barcelona OpenMP Task Suite: NQueens~\cite{5361951}.
%In this problem, $n$ queens must be placed on a board of size $n x n$ without threatening each other. The task based algorithm proceeds row-wise by trying to place a queen on each column of a given row. New tasks are spawned for each placement that could lead to a solution.  
%For NQueens for example, the total work is $O(n!)$, the depth of the task graph is $n$.~\cite{10.1145/3155284.3018770}. For the first rows, the number of tasks is small. However, the explosive growth makes \toolname efficient as early as the Xth row.
As an example, we consider the prefix scan in electron microscopy
image registration~\cite{copik2020workstealing}.
%
The width of the task graph in a distributed scan varies significantly between program phases,
affecting the parallel efficiency. %parallelism and its efficiency.
%
The dispatch of tasks expands parallel resources only when needed
and limits the static resource allocation to the most efficient configuration.
%\lex{Here we need also need to add an actual example - Let's assume hot invocations, and whatever a benchmark he choose has as a payload, but here we should show a small part of the TDG and what can be offloaded at 2 different points.}

% NEGATIVE VSPACE
\ifcnf
\vspace{-0.75em}
\fi
\paragraph{Hybrid BSP Applications}
%
%\hl{A more complex case is an application that uses MPI
%and a shared-memory parallel programming framework, e.g., OpenMP.
%%
%This is a common occurrence in HPC, and we propose 
%to boost the performance of such applications using \toolname{}. 
A common occurrence in HPC are applications
that use MPI and a shared-memory parallel programming framework, e.g., OpenMP,
and we propose to boost the performance of such programs using \toolname{}. 
%
We assume a bulk synchronous execution at the MPI level: each
rank performs mostly the same type of computation.
%
In this case, we consider candidates for remote invocations
OpenMP parallel loops or task constructs with no shared accesses.
%
By applying Eq.~\ref{eq:offload}, we can determine how many
loop iterations or tasks can be safely offloaded without incurring waiting times.
%
Even if a small number of iterations or tasks are solved remotely, this
can still amount to significant computational effort in total,
as \emph each MPI process performs the same amount of work.

Since \toolname{} has finite resources, the application
must handle the case of \emph{resource starvation}.
%
While this is an application-specific problem, we provide a general principle of resource-aware
serverless acceleration for BSP programs presented in Figure~\ref{fig:rfaas_bsp}.
%
In addition to \emph{public} executors offered by the \toolname{} service,
MPI processes run \emph{private} executors that allow for job-internal offloading.
%
Thanks to the rigid structure of bulk synchronous computations, MPI ranks can mutually exchange
their acceleration status before entering computational loops
and find acceleration partners offering private executors.
%
This technique allows to load-balance by distributing the workload across
the entire MPI application with a single, consistent interface of serverless functions.
%
Thus, load-balancing is possible even in case of full saturation
and unequal resource availability.

%Let us look at the LULESH proxy app as an example. Considering the OpenMP loop in the IntegrateStressTermsForElems function, the loop is iterated once for each element in the physical domain, and each iteration performs 463 floating point operations.
%\lex{same story, we need the numbers here once we have them}




==> secs/evaluation.tex <==
\label{sec:evaluation}
To demonstrate \toolname{} fitness for HPC,
we answer critical questions in the form of extensive evaluation.

\begin{enumerate}[noitemsep,nosep]
\item Is \toolname fast enough for latency-sensitive, high-performance applications?
\item Are the overheads for initialization prohibitively large?
\item Does \toolname{} bandwidth scale with larger payloads?
\item Does \toolname{} scale with more parallel workers?
%\item Does \toolname{} allocations scale with more workers?
%\item Do faster invocations benefit more from RDMA or decentralization?
\item Does \toolname{} help to integrate functions into latency-sensitive applications?
%\item Does \toolname{} improve performance for typical high-performance applications?
\item Is the performance of remote computing with \toolname{} competitive when compared to local computation?
\item Are short \toolname{} functions usable in HPC computations?
\end{enumerate}

\paragraph{Platform}
%
We deploy \toolname{} in a local cluster and execute benchmark code on 4 nodes,
each with two 18-core Intel(R) Xeon(R) Gold 6154 CPU @ 3.00GHz and 377 GB of memory.
%
Nodes are equipped with Mellanox MT27800 Family NIC with a 100 Gb/s Single-Port link that
is configured with RoCEv2 support.
%
Nodes communicate with each other via a switch,
%
% RDMA 1, p50 3.6933800000000003, p95 3.72278, p99 3.7394800000000004
and we measured an RTT latency of 3.69 $\mu$s and a bandwidth of 11,686.4 MiB/s.
%
We use Docker 20.10.5 with the executor image \texttt{ubuntu:20.04},
and we use the Mellanox's SR-IOV plugin to run containers over virtual device functions.
%
\toolname is implemented in C++, using g++ 8.3.1. MPI benchmarks are implemented using OpenMPI 4.0.5.

\subsection{Invocation Latency}
%
\begin{figure}[tbh!]
	\centering
  \includegraphics[width=1.0\linewidth]{figures/evaluation_hot_warm}
  \vspace{-1em}
  \caption{The RTT of an no-op \toolname{} function and network transport,
  median (solid) and 99th latency (dashed).}
  \label{fig:evaluation_hot_warm}
\end{figure}

%\copik{Add Azure IB results, add results for Knative, fission}

%\textbf{Hypothesis:} \toolname supports function invocations with less than 300 ns overhead.

%netperf - buffer + alignment + offsets, CPU thread pinning, reported mean, 1 iteration
%perftest - warmup iters, reported median, CPU thread pinning

We begin with the most important characteristic for \toolname:
the latency of invoking a remote function.
%
%We measure hot and warm invocations of empty functions that accept input of a given size,
%and return the same amount of data.
We measure hot and warm invocations of a non-op ''echo'' function that returns the provided input.
%
We use a warmed-up, single-threaded, bare-metal executor with the main thread pinned to a CPU core,
perform 10,000 repetitions, and report the median.
%
We compute the non-parametric 99\% confidence intervals of the median~\cite{10.1145/2807591.2807644,le2010performance}, and find that the interval bounds are very tight ($<1\%$).
%
To assess the overheads of \toolname invocations, we measure the latency
of RDMA and TCP/IP transmissions. %on the same network device.
%
For the former, we use \emph{ib\_write\_lat} from the \emph{perftest} package,
execute it with thread pinning and warm-up iterations, and report the median.
%
For the latter, we use \emph{netperf} with page-aligned buffers and process
pinning, and report the mean.

Fig.~\ref{fig:evaluation_hot_warm} shows
that the overhead imposed by processing a no-op function by \toolname{} in a process is 326 ns on average when compared to the baseline data transmission with RDMA writes.
%
The measurements for a Docker-based executor present aditional ca. 50 ns overhead over RDMA writes
when using a container.
%
The only exception is the message size of 128 bytes, where the overhead increases to 630 ns.
There, RDMA can use message inlining for both directions of the transmission which improves
 the performance of small messages significantly~\cite{anujKVS}.
%
However, the communication in \toolname is asymmetrical: we transmit 12 bytes more for
the input. The maximal supported inlining size is 128 bytes on our device,
forcing \toolname to use non-inlined write operations for one direction.
%
The average overhead of a warm execution is 4.67 $\mu$s.
%
Here, the containerization adds a measurable overhead, and Docker-based warm
executions have an additional latency of ca. 650 ns. %nanoseconds.

With slightly more than 300 ns of overhead, \toolname enables remote invocations with
no noticeable performance penalty, conclusively answering: \textbf{\toolname is fast enough for  latency-sensitive, high-performance applications}.

\begin{figure}[tbh!]
	\centering
  \resizebox*{0.95\width}{0.92\totalheight}{
    \subfloat[Bare-metal Linux process
    ]{%	
      \includegraphics[width=1.0\linewidth]{figures/cold_baremetal}\label{fig:cold_baremetal}
    }
	}
	\hfill
	\resizebox*{0.95\width}{0.92\totalheight}{
		\subfloat[Docker container
		]{%	
      \includegraphics[width=1.0\linewidth]{figures/cold_docker}
      \label{fig:cold_docker}
		}
	}
  \vspace{-1em}
  \caption{Cold invocations of \toolname functions.}
  %\vspace{-1em}
\end{figure}

\subsection{Cold Invocation Overheads}
%The next question we tackle is that of initialization overhead.
Fig.~\ref{fig:cold_baremetal} and~\ref{fig:cold_docker} present the overhead of a single \emph{cold}
invocation on a bare-metal and Docker-based executor, respectively.
The data comes from 1000 invocations with a single no-op C++ function, compiled into
a shared library of size 7.88 kB.
%
In all tested configurations, the longest step is the creation of workers. 
%
All other steps: the connection establishment to the manager, submitting an allocation and code,
and code invocation, take single-digit milliseconds to accomplish.
%
We can therefore claim that \toolname{} does not introduce significant overheads apart from the sandbox initialization.

While the current version of Docker shows an overhead of approximately 2.7 seconds to spawn workers,
low-latency approaches such as Firecracker~\cite{246288} reduce this time to as little as 125 milliseconds.
%
Furthermore, \toolname{} puts no new requirements on the sandbox system except for network device virtualization.
%
Thus, it is compatible with proposed approaches for reducing cold startup latencies, such as container warming and reinitialization~\cite{234835,7979855}.
%
Finally, the user's function can be deployed as a code package like in many other FaaS platforms, allowing executor managers to keep a pool of generic and ready containers and bypass the startup latencies of the Docker container.
%
%Firecracker cannot currently deploy on HPC systems, but the developers are working towards expanding its capabilities. 
 
In HPC applications, the initialization time of MPI takes between 0.8 and 3 seconds for 32 processes
depending on the MPI library used~\cite{10.1007/978-3-540-30474-6_47} --- comparable to the \toolname{}
overhead of cold initialization.
%
%Developers can overcome this overhead by initializing \toolname like
%calling \textit{MPI\_Init()}: as soon as the application starts.
%%
%The nonblocking nature of this initialization should allow \toolname workers to be ready to
%receive code by the time they complete their own initialization.
Developers can overcome this overhead by initializing \toolname like
calling \textit{MPI\_Init()}, and the nonblocking nature of this
process should allow \toolname workers to be ready to
by the time MPI completes its own initialization.

We therefore claim that \textbf{cold invocation overheads of \toolname do not pose an obstacle for the use in HPC}.
%Research question: how our manager-based scheme compares with the AWS API Gateway and OpenWhisk
%invocation?

\subsection{Bandwidth scalability}
\label{sec:evaluation_payload}

To compare the performance of \toolname and other platforms, %with respect to payload sizes,
we evaluate a non-op C++ function that returns the provided input on a payload range from 1 kB to 5 MB.
%
Since other platforms cannot accept raw data, we generate a base64-encoded
string that approximately matches the input size used in \toolname.
%
%We compare against: AWS Lambda~\cite{awsLambda}, a state-of-the-art,
%popular commercial FaaS solution.
%
%Then, we compare against Nightcore~\cite{nightcore}, a low-latency FaaS platform,
%and OpenWhisk~\cite{openwhisk}, an open-source FaaS platform.
%
%%
%We deploy the platform on the cluster, create a no-op C++ function, and invoke it
%from another machine.
%}
%%
%Finally, we compare against OpenWhisk~\cite{openwhisk}, an open-source FaaS platform.
%%
%We deploy a standalone OpenWhisk using Docker with Kafka and API gateway~\cite{openwhiskDocker},

%%
%In this case, the function is implemented using the official C++ Runtime for AWS Lambda~\cite{awsCRuntime} and deployed as a native function.
%%
%We expose an HTTP endpoint with no authorization, and rent an AWS \emph{t2.micro} virtual
%machine instance in the same region as the function to measure the invocation latency for the 
%provided endpoint.
%%
%\marginpar{\hspace{35em}\colorbox{orange}{\textbf{REV-1}}}
%\marginpar{\hspace{35em}\colorbox{orange}{\textbf{REV-5}}}
%\hl{
%Then, we compare against Nightcore~\cite{nightcore}, a low-latency FaaS platform.
%%
%We deploy the platform on the cluster, create a no-op C++ function, and invoke it
%from another machine.
%}
%%
%Finally, we compare against OpenWhisk~\cite{openwhisk}, an open-source FaaS platform.
%%
%We deploy a standalone OpenWhisk using Docker with Kafka and API gateway~\cite{openwhiskDocker},
%%
%create a native action and invoke it through the provided URL.
%%from a remote server.
%%
%A C++ function in OpenWhisk is invoked as a regular application, accepting input
%through \emph{argc} and \emph{argv}, but does not accept inputs > 125 kB.
\iftr
We compare against AWS Lambda~\cite{awsLambda}, a state-of-the-art commercial FaaS solution,
as Azure Functions~\cite{azureFunctions} and Google Cloud Functions~\cite{googleFunctions}
do not support C++ functions.
%
Then, we compare against open-source FaaS platforms OpenWhisk~\cite{openwhisk},
and Nightcore~\cite{nightcore}, a low-latency and open-source serverless platform.
\else
We compare against AWS Lambda, a state-of-the-art commercial FaaS solution,
as neither Azure Functions nor Google Cloud Functions support C++ functions.
%
Then, we compare against open-source FaaS platforms OpenWhisk
and Nightcore~\cite{nightcore}, a low-latency and open-source serverless platform.
\fi
%
Both open-source systems are deployed on the same RDMA-capable cluster as \toolname{}, using the same network and CPU
resources as our system.
%
\iftr
In Lambda, we deploy a native function implemented using the official C++ Runtime~\cite{awsCRuntime},
we expose an HTTP endpoint with no authorization, and run the experiment in
an AWS \emph{t2.micro} VM instance in the same region as the function.
%
We deploy on the cluster a standalone OpenWhisk using Docker with Kafka and API gateway~\cite{openwhiskDocker}.
\else
In Lambda, we deploy a native function implemented with the C++ Runtime,
we expose an HTTP endpoint with no authorization, and run the experiment in
an AWS \emph{t2.micro} VM instance in the same region as the function.
%
We deploy on our cluster a standalone OpenWhisk using Docker with Kafka and API gateway.
\fi
%
A C++ function in OpenWhisk is invoked as a regular application, accepting inputs no larger than 125 kB
through \emph{argc} and \emph{argv}.
%
We deploy a \emph{nightcore} instance on the cluster with a non-op C++ function.

We present the evaluation result in Fig.~\ref{fig:evaluation_faas} (page 1).
%
On all payload sizes, \toolname clearly provides significantly better performance.
%
\toolname invocations are between 695x and 3,692x faster than AWS Lambda executions,
thanks to the performance attainable with a low-latency network
and the native support for transmitting raw data that suits high-performance applications very well.
%
\toolname{} is between 23x and 39x times faster than Nightcore, another FaaS platform
with microsecond-scale latencies.
%
Similarly, \toolname provides a speedup between 5,904x and 22,406x when compared to OpenWhisk.

Therefore, we answer that \toolname provides significant performance improvements over contemporary FaaS platforms and \textbf{\toolname scales well with message size}.

%\begin{figure}[tbh!]
%	\centering
%  \resizebox*{0.95\width}{0.92\totalheight}{
%    \subfloat[1 kB message
%    ]{%	
%      \includegraphics[width=1.0\linewidth]{figures/evaluation_parallel_1024}\label{fig:parallel_1024}
%    }
%	}
%	\hfill
%	\resizebox*{0.95\width}{0.92\totalheight}{
%		\subfloat[1 MB message
%		]{%	
%      \includegraphics[width=1.0\linewidth]{figures/evaluation_parallel_1048576}
%      \label{fig:parallel_1M}
%		}
%	}
%  \caption{\toolname invocations on parallel executors.}
%\end{figure}

\begin{figure}[tbh]
	\centering
  \includegraphics[width=0.98\linewidth]{figures/parallel_combined}
  \vspace{-0.5em}
  \caption{\toolname invocations on parallel executors.}
  %\vspace{-2em}
  \label{fig:parallel_combined}
\end{figure}

\subsection{Parallel scalability}
\label{sec:evaluation_parallel}

To verify that RDMA-capable functions scale efficiently to handle integration
into scalable applications, we place managers on 36-core CPUs
%and evaluate the overheads
and evaluate parallel invocations. 
%
We execute the no-op function on warmed-up, bare-metal executors having allocated from 1 to 32
worker threads.

Fig.~\ref{fig:parallel_combined} presents the round-trip latencies
for invoking functions with 1 kB and 1MB payloads, respectively.
%
The overhead of handling many concurrent connections is insignificant on hot invocations
with a smaller payload.
%
While the Docker executor shows performance increase (hot) and decrease (warm)
on the 1 kB payload, the difference on 1MB payload is less than 1\%.
%
However, execution times increase significantly with the number of workers when sending
1 MB data, due to saturating network capacity (100 Gb/s).
This shows that \toolname scaling is limited only by the available bandwidth.
%explained by comparing against the measured bandwidth of the RDMA device by plotting
%the time needed for the round-trip transport of the payload to each worker.
%The comparison shows the 

Therefore, we claim that \textbf{parallel scaling of \toolname{} executors is bounded only by network capacity}.

\begin{figure}[tbh!]
	\centering
  \subfloat[Image processing: thumbnail generation: \emph{AWS Lambda} and \emph{\toolname{}}.]{
    \includegraphics[width=1.0\linewidth]{figures/faas_benchmark_image_thumbnailer}
    \label{fig:faas_thumbnailer}
  }
  \vspace{-1em}
  \hfill
  \subfloat[Image recognition with ResNet-50 and PyTorch: \emph{AWS Lambda}, \emph{\toolname{}}.]{
    \includegraphics[width=1.0\linewidth]{figures/faas_benchmark_image_recognition}
    \label{fig:faas_recognition}
  }
  \vspace{-1em}
  \caption{\toolname{} on serverless functions, reported medians with parametric 99\% CIs.}
  %\vspace{-1em}
\end{figure}

%\subsection{RDMA vs Decentralized Allocation.}
%\copik{Add experiment where we run the new port with TCP provider - compare latency.}
%\copik{Add experiment with "gateway" with double latency and RDMA - compare latency.}

\subsection{Use-case: serverless functions}
%\vspace{-0.5em}
To evaluate the effectiveness of \toolname{} in integrating serverless functions
into high-performance applications, we select real-world serverless functions from the SeBS benchmark~\cite{copik2021sebs}.
%
We take the \emph{thumbnailer} benchmark as an example of general-purpose image processing
and the \emph{image-recognition} benchmark performing ResNet-50 prediction as an example of integrating
deep-learning inference into applications.
%
We reimplement the Python benchmarks in C++ and deploy them as Docker images on \toolname{}
and AWS Lambda.
%, as the C++ dependencies are too large for the Lambda code package.
% with a size limit of 250 MB.
%
%For the latter, we use the official C++ Runtime~\cite{awsCRuntime} and the Docker image for 
%provided runtimes.
%
We repeat each benchmark 100 times.
\paragraph{Image processing}
%
We implement the thumbnail generation with OpenCV 4.5.
%
We evaluate functions with two images, 97 kB \emph{small} one and a 3.6 MB \emph{large} one 
(Fig.~\ref{fig:faas_thumbnailer}).
%
For the AWS Lambda function, we need to submit the binary image data as a base64-encoded string
in the POST request, which adds significant performance overheads due to encoding and conversions.
%
Furthermore, 
%
On the other hand, \toolname{} functions benefit from the payload format
%that is
not constrained by cloud API requirements.
%
\paragraph{Image registration}
%
We implement the benchmark with the help of PyTorch C++ API, using \emph{OpenCV} 4.5, \emph{libtorch}
1.9, and \emph{torchvision} 0.1.
%
We convert the Python serialized model included with \emph{SeBS} into the recommended TorchScript model format.
%
The model is included with the Docker image and stored in the function memory after the first invocation.
%
We evaluate functions with two inputs, a 53 kB \emph{small} image and a 230 kB \emph{large} one 
(Fig.~\ref{fig:faas_recognition}).
%
There is a growing interest in using machine-learning inference to speed up computations and
simulations~\cite{brace2021achieving,10.3389/fdata.2020.604083,Krupa_2021}.
%
The results demonstrate that \textbf{\toolname{} functions can efficiently implement inference
tasks in high-performance applications}.

%In both cases, \toolname{} outperforms AWS Lambda on large memory allocations that receive more than one virtual CPU in the cloud.
%
%The results demonstrate that invocation add significnt \textbf{\toolname{} functions can efficiently implement inference
%tasks in high-performance applications}.

\begin{figure}[tbh!]
  \centering
  %\hfill
  %\subfloat[Black-Scholes from PARSEC 3.0, 10 million equations: \emph{OpenMP}, \emph{\toolname{}}.]{
  \includegraphics[width=1.0\linewidth]{figures/blackscholes_native.pdf}
  \vspace{-1.5em}
  \caption{Parallel serverless computing with \toolname{} and \emph{OpenMP}. Reported medians with non-parametric 95\% CIs.}
  %\vspace{-1em}
  \label{fig:blackscholes}
  %}
  %\caption{Parallel serverless computing with \toolname{}, reported medians with non-parametric 95\% CIs.}
\end{figure}

\subsection{Use-case: parallel offloading}
%
We want to answer the next question: can \toolname{} offload computations efficiently to remote serverless workers?
%
To answer this question, we study offloading of massively parallel computations with significant data movement.
%
We select the Black-Scholes solver~\cite{10.1080/00207160.2012.690865} from the
PARSEC suite~\cite{10.1145/1454115.1454128} parallelized with OpenMP threading.
%
Black-Scholes solves the same partial differential equation for different parameters,
and we dispatch independent equations to bare-metal parallel executors.
%
We evaluate the benchmark %on \emph{native} input with approximately 229 MB of input and 38 MB of output
with approx. 229 MB of input and 38 MB of output
and present results in Fig.~\ref{fig:blackscholes}.
%
%In this benchmark, the ratio of computation to communication is low, which emphasizes the need to efficiently

We show that offloading the entire work to \toolname{} scales efficiently compared to OpenMP,
as long as the workload per thread is not close to the network transmission time of approximately 20 ms.
%
We can further speed the OpenMP application up by offloading
half of the work to the same number of serverless functions (\emph{OpenMP + }\toolname{}).
%
Since other high-performance FaaS systems achieve a fraction of available bandwidth (Sec.~\ref{sec:evaluation_payload}),
their runtime will be dominated by the transmission of 229MB of data to functions.
%
\textbf{Thus, we can conclude that \toolname{} offers scalable parallelism bounded by network performance only.}

\begin{figure}[tbh!]
 \centering
  \subfloat[Matrix-matrix multiplication: \emph{MPI} (dashed) and \emph{MPI+\toolname{}} (solid).]{
    \includegraphics[width=0.49\linewidth]{figures/mat-mat}
    \label{fig:res_mmm}
  }
  %\hfill
  \subfloat[Jacobi method, 100 iterations: \emph{MPI} (dashed) and \emph{MPI+\toolname{}} (solid).]{
    \includegraphics[width=0.49\linewidth]{figures/jacobi_plot}
    \label{fig:res_jacobi}
  }
  \vspace{-1em}
  \caption{\toolname{} in practice, reported medians with non-parametric 95\% CIs.}
  %\vspace{-2em}
\end{figure}

%\begin{figure}[tbh!]
% \centering
%  \subfloat[Matrix-matrix multiplication: \emph{MPI} (dashed) and \emph{MPI+\toolname{}} (solid).]{
%    \includegraphics[width=1.0\linewidth]{figures/matrix_size_new2}
%    \label{fig:res_mmm}
%  }
%  \hfill
%  \subfloat[Jacobi method, 100 iterations: \emph{MPI} (dashed) and \emph{MPI+\toolname{}} (solid).]{
%    \includegraphics[width=1.0\linewidth]{figures/matrix_size2}
%    \label{fig:res_jacobi}
%  }
%  \caption{\toolname{} in practice, reported medians with non-parametric 95\% CIs.}
%\end{figure}

\subsection{Use-case: HPC Applications}
%
%The HPC world is dominated by the Message-Passing Interface (MPI) programming model,
%a \emph{de facto} standard distributed programming paradigm.
%
%In the rigid HPC world, \emph{evolving} and \emph{malleable} applications~\cite{10.1007/BFb0022284}
%use only a fixed number of resources that cannot be easily adjusted,
%leading to overallocation and underutilization of cores on computations with irregular parallelism.
%
%Sadly, the question of incorporating elastic cloud resources into high-performance applications
%remains open due to a lack of a cloud-native programming model.

The next question we want to answer is: how much performance can be gained by offloading
complex tasks to the cheap and spare capacity of HPC clusters?
%%
%To find an answer, we use a matrix-matrix multiplication kernel as a stand-in for compute-intensive
%tasks in general,
%To learn how much efficient offloading complex tasks to the cloud can be,
%we use a matrix-matrix multiplication kernel as a stand-in for compute-intensive tasks in general,
%and compare the performance of a traditional MPI application with an \emph{elastic} one that
%uses \toolname{} acceleration.

\paragraph{Matrix-matrix multiplication}
\label{sec:eval-mat-mat}
%
We run an \emph{MPI} application where each rank performs a matrix-matrix multiplication,
averages it over 100 repetitions, and we measure the median kernel time across MPI ranks.
%
MPI ranks are distributed across two 36-core nodes, and we pin each rank to a single core.
%
Then, we deploy an \emph{MPI + rFaaS} application where each rank allocates a single bare-metal
\toolname{} function.
%
\toolname{} executors are deployed on two other 36-core nodes, and with such concentration
of MPI and \toolname{} computing resources, we show that sharing the network bandwidth does not
prevent efficient serverless acceleration.
%
Because of a high computation to communication ratio,
we split workload equally, and both MPI rank and the function compute half of the result matrix.
%
Figure~\ref{fig:res_mmm} shows \toolname provides a speedup between
1.88x and 1.94x depending on the number of MPI processes.
%
%This speedup is consistent as we vary the size of the multiplied matrices.
%
%We implemented the same function on the Nightcore FaaS platform.
%
%As functions there accept only JSON arguments,
%we serialize matrices with C++ libraries~\cite{cerealLib,tencetJSON}.
%
%We deployed two instances with a fixed number of 32 function instances,
%and performed the same evaluation.
%
%The \emph{MPI + nightcore} achieves worse speedup due to the overhead of serialization,
%and lower utilization of network bandwidth.
%
Functions with a good ratio of computation to unique memory accesses can
be accelerated with \toolname. As long as this condition holds,
\textbf{\toolname improves the performance of HPC workloads}.

\paragraph{Jacobi linear solver}
To show a serverless acceleration of a bulk synchronous type of problem,
we consider the Jacobi linear solver,
where half of each iteration is offloaded to \toolname{}.
%
Here, we perform a classical serverless optimization of caching resources in a warmed-up
sandbox.
%
Since the matrix and right-hand vector do not change between iterations, we submit
them only for the first invocation.
%
As long as the allocated function is not removed, we send only
an updated solution vector in consequent iterations.

We evaluate the approach in the same setting as matrix multiplication (Section~\ref{sec:eval-mat-mat}),
with MPI ranks averaging Jacobi method with 1000 iterations over ten repetitions and measured a speedup between 1.7 and 2.2 when \toolname{}
acceleration is used.
%
Since each iteration takes just between 1 and 15 milliseconds,
results must be returned with a minimal overhead
to offer performance comparable with the main MPI process:
%
\textbf{the low-latency invocations in \toolname{} apply to millisecond-scale computations.}

%\subsubsection{Black-Scholes}
%We show how \toolname{} can accelerate a pure OpenMP application,
%using the Black-Scholes solver~\cite{10.1080/00207160.2012.690865} from the
%PARSEC suite~\cite{10.1145/1454115.1454128}.
%
%Black-Scholes solves the same partial differential equation for different parameters,
%and we dispatch independent equations to bare-metal parallel executors.
%
%We evaluate the benchmark on \emph{native} input with approximately 229 MB of input and 38 MB of output
%and present the results in Figure~\ref{fig:blackscholes}.
%
%We show that offloading the entire work to \toolname{} scales efficiently compared to OpenMP,
%as long as the workload per thread is not close to the network transmission time of approximately 30 ms.
%
%We achieve further speedup by enhancing the OpenMP application with offloading
%half of the work to the same number of parallel workers cloud resources.
%
%\textbf{\toolname{} offers scalable parallelism bounded by network performance only.}



